Distributional Generalization: A New Kind of Generalization

We introduce a new notion of generalization -- Distributional Generalization -- which roughly states that outputs of a classifier at train and test time are close *as distributions*, as opposed to close in just their average error. For example, if we mislabel 30% of dogs as cats in the train set of CIFAR-10, then a ResNet trained to interpolation will in fact mislabel roughly 30% of dogs as cats on the *test set* as well, while leaving other classes unaffected. This behavior is not captured by classical generalization, which would only consider the average error and not the distribution of errors over the input domain. Our formal conjectures, which are much more general than this example, characterize the form of distributional generalization that can be expected in terms of problem parameters: model architecture, training procedure, number of samples, and data distribution. We give empirical evidence for these conjectures across a variety of domains in machine learning, including neural networks, kernel machines, and decision trees. Our results thus advance our empirical understanding of interpolating classifiers.

==> app_general.tex <==
\section{Generalized Generalization: Appendix}
\label{sec:app-general}

==> app_more_discuss.tex <==
\section{More Discussion}

\pnote{scratch section for now}

The 1-nearest-neighbor mechanism is consistent with
many of the other behaviors we observe in this work,
and we prove that these behaviors would occur for 1-NN.
The specific choice of 1-NN is not critical here,
and we may generally expect such behaviors
from \emph{local} estimators where
the classification at a test point is 
primarily determined by identifying it
with a corresponding train point
(for example, Nadaraya-Watson kernel smoothers
with a suitably sharp kernel).
However, it is surprising that we observe these behaviors
for neural-networks and kernel regressors,
which are typically not considered ``local'' estimators.
\pnote{Add that this isn't about label noise specifically}

\textbf{Connection between density estimation and classification:} If we have a good way to get a good density estimate $f(x) = p(y|x)$, it is trivial to obtain a good classification from it $\hat{y} = \argmax f(x)$. On the other hand, our conjecture highlights a novel connection between classification and density estimation in the opposite direction --- when a classifier is trained to interpolation, the output distribution $(x, f(x))$ of this classifier is close to the input distribution $(x, y)$ in an $\emph{approximate}$ sense, even thought it is not trained for this purpose. Specifically, if a distinguishable partition of the domain has different label density for each of the $M$ parts, the interpolated classifier will match the label density for each of these parts. 

\pnote{incorporate this somehow:}
We find it surprising that even when the dataset contains a large fraction of dogs in cats' skin, the network continue to classifies the cats accurately, and mislabels the dogs in the \emph{right} proportion. This suggests that the effect of this mislabelling is \emph{localized} to the dogs. 








==> app_student.tex <==
\section{Student-Teacher: Appendix}
\label{sec:app-student}

\subsection{Experimental Details}

\paragraph{Setup.}
Throughout this section, we use ResNet18
for all networks (students and teachers).
We first train several teacher networks $\{F_n\}$
for CIFAR-10,
by randomly subsampling
the first half of the CIFAR-10 train set
to
$n=\{1000, 2000, 5000, 10000, 15000, 25000\}$
train samples.
\pnote{todo: redo this with exponential spacing}
We then evaluate these networks on the second half of the CIFAR-10 train set (denoted by $S$),
to obtain pseudo-labeled train sets $\{S, F_n(S)\}$.
Finally, for each $k, n \in \{1000, 2000, 5000, 10000, 15000, 25000\}$,
we train a student network $G_{n, k}$ on $k$ random pesudo-labeled samples from $(S, F_n(S))$.

We then evaluate the test errors $E(n, k) := \textrm{TestError}_\cD(G_{n, k})$
via the CIFAR-10 test set.

\subsection{Results}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/st_grid.png}
    \caption{todo.}
    \label{fig:st_grid}
\end{figure}

As an aside, notice that the test error appears to $G_{n,k}$ depend only on $\min(n, k)$.
Intuitively, the test error is bottlenecked by the minimum power of student and teacher.


==> intro6.tex <==
\section{Introduction}
In this paper we introduce a new notion of generalization,
which sheds light on the behavior of standard classification methods.
We motivate this notion via extended examples
in Section~\ref{intro:motiv},
which highlight the limitations of classical generalization and the breadth of our results.
In the Introduction, we first discuss the mathematical form of classical generalization, to set the stage for our extension.
We then informally discuss our concrete conjectures
and summarize our contributions in the remainder of the paper.


\subsection{Classical Generalization}

The goal of supervised learning for classification is to learn a model that correctly classifies inputs $x \in \cX$ from a
given distribution $\cD$ into classes $y \in \cY$.
We want a model with small \emph{test error} on this distribution.
In practice, we find such a classifier by minimizing
a proxy quantity: the \emph{train error} of a model on the train set.
The classical framework for supervised learning, empirical risk minimization,
says that this procedure is justified
when the model output by the learning algorithm is expected to have
a small \emph{generalization gap}: the gap between the error on the train and test set.
Formally, the trained model $f$ should be such that:
\begin{align}
\textrm{Error}_{\textrm{TrainSet}}(f)
\approx
\textrm{Error}_{\textrm{TestSet}}(f)
\end{align}

This states that the model's behavior on the test set is similar to its behavior on the train set,
as measured by the error.
In our work we extend this notion of generalization, and show that 
models behave similarly on the train and test sets
in more ways than just their error.

To make this clearer, we first re-write the classical notion of generalization given in Equation (1) in a form better suited for our extension.

{\bf Classical Generalization:}
{\it
Let $f$ be a classifier trained on a set of samples (\TrainSet).
Then $f$ generalizes if:
\begin{align}
\label{eqn:classic}
\E_{\substack{
x \sim \TrainSet\\
\hat y \gets f(x)
}}
[
\1\{\hat{y} \neq y(x)\}
]
\approx
\E_{\substack{
x \sim \TestSet\\
\hat y \gets f(x)
}}
[
\1\{\hat{y} \neq y(x)\}
]
\end{align}
where $y(x)$ is the true class of $x$, and $\hat{y}$ is the predicted class.
}

The LHS of Equation~\eqref{eqn:classic} is the train error of $f$, and the RHS is the test error.
Crucially, both sides of Equation~\eqref{eqn:classic}
are expectations of the \textit{same function}--- the error function---
under \textit{different distributions}.
The error function 
$$\Terr(x, \hat y) :=  \1\{\hat{y} \neq y(x)\}$$
indicates whether the classifier output $\hat{y}$ agrees with the true label of $x$. 

The LHS of Equation (2) is the expectation of
$\Terr$
under the ``Train Distribution'', which
is the distribution over $(x, \hat{y})$ given by sampling a train point $x$
along with its classifier-label $f(x)$.
Similarly, the RHS is under the ``Test Distribution'', which is this same construction over the test set:

\begin{enumerate}
    \item $\textrm{Train Distribution $\Dtr$: } (x, f(x))_{x \sim \TrainSet}$
    \item $\textrm{Test Distribution $\Dte$: } (x, f(x))_{x \sim \TestSet}$
\end{enumerate}

These two distributions are the central objects in our study. Classical generalization requires that these two distributions are close
with respect to a specific statistical functional: the expectation of the error function.

However, expected error is only one statistic that could match between these two distributions.
In this work, we show that the train and test distributions are close in many other statistics, which we formally characterize.
Moreover, we show that many statistics match even when the test error itself does not match --
that is, when the generalization gap is high.
This includes settings when training data is limited, the data is noisy or randomized, or the classification task is hard. 









\subsection{Distributional Generalization}
\label{sec:intro-dgen}

We frame our results via a natural extension of classical generalization,
which we call ``Distributional Generalization.''
Distributional Generalization is a property of trained classifiers, similar to classical generalization.
It is parameterized by $\mathcal{T}$, a set of bounded functions (``tests'') from $\cX \x \cY$ to $[0, 1]$:
$$
\mathcal{T} \subseteq \{T: \cX \x \cY \to [0, 1]\}
$$


{\bf Distributional Generalization:}
{\it 
Let $f$ be a classifier trained on \textrm{TrainSet}.
Then $f$ satisfies Distributional Generalization with respect to tests $\cT$ if:
\begin{align}
\forall T \in \mathcal{T}:
\quad
\E_{\substack{
x \sim \textrm{TrainSet}\\
\hat y \gets f(x)
}}
[
T(x, \hat{y})
]
\approx
\E_{\substack{
x \sim \textrm{TestSet}\\
\hat y \gets f(x)
}}
[
T(x, \hat{y})
]
\end{align}
which we also write as
\begin{align}
\label{eqn:intro-dg}
\Dtr \approx^{\cT} \Dte
\end{align}
}

This property states that the train and test distribution have
similar expectations for all functions in the family $\mathcal{T}$.
For the singleton set $\cT = \{\Terr\}$, this is equivalent to classical generalization.
However $\cT$ can be much larger -- and in this work we conjecture
that Distributional Generalization often holds for a large family $\cT$ which we specify later.
In fact, we will see that
the family of functions $\mathcal{T}$ is often so large that is
it is best to think of Distributional Generalization
as stating that the distributions $\Dtr$ and $\Dte$
are close \emph{as distributions} (as suggested by the notation of Equation~\eqref{eqn:intro-dg}, made formal
in Section~\ref{sec:dist-closeness}).

This property becomes especially interesting 
for \emph{interpolating classifiers}, 
which fit their train sets exactly.
Here, notice that the Train Distribution $\Dtr$
is exactly equal\footnote{The formal definition of Train Distribution, in Section~\ref{sec:general}, includes the randomness of sampling the train set as well.
We considered a fixed train set in the Introduction for sake of exposition.} to the original distribution $\cD$,
since $f(x_i) = y_i$ on the train set.
In this case, distributional generalization claims that the
output distribution $(x, f(x))$ of the model on test samples
is close to the \emph{true} distribution $(x, y)$.



The following conjecture specializes Distributional Generalization
to interpolating classifiers, and will be the main focus of our work.




\begin{boxedenv}{\bf Interpolating Indistinguishability Meta-Conjecture (informal):}

{\it 
Let $f$ be an interpolating classifier trained on \textrm{TrainSet}.
Now, for a large family $\mathcal{T}$ of statistical tests depending on $f$ (to be specified later):
\begin{align}
\label{eqn:metaconj}
\cD \equiv \Dtr \approx^{\cT} \Dte
\end{align}
}

{\normalfont We state this conceptually as }
{\it
``For interpolating classifiers $f$:
The distributions $(x, y)$ and $(x, f(x))$
on the test set look the same
to a certain family of tests''
}
\end{boxedenv}


This is a ``meta-conjecture'', which becomes a concrete conjecture
once the family of tests $\mathcal{T}$ is specified.
One of the main contributions of our work
is formally stating two concrete instances of this conjecture---
specifying exactly the family of tests $\mathcal{T}$
and their dependence on problem parameters 
(the distribution, model family, training procedure, etc).
We empirically verify these conjectures across a variety of natural settings
in machine learning.
These experiments themselves highlight new behaviors of interpolating classifiers
which are independently interesting.

In the remainder of the Introduction we will discuss the two concrete conjectures, Feature Calibration
and Agreement Matching, which form the two main sections in the body of our paper
(Sections~\ref{sec:dist-features} and~\ref{sec:agree}).
We start with several examples, then discuss the conjectures
in Sections~\ref{intro:feat} and \ref{intro:agree}.
We conclude by discussing potential mechanisms
and summarizing our contributions.

\subsection{Motivating Examples}
\label{intro:motiv}
We now present several experiments which motivate the need for
a notion of generalization beyond test error.

\begin{experiment}
\label{exp:intro1}
Consider a binary classification version of CIFAR-10,
where CIFAR-10 images $x$ have binary labels \texttt{Animal/Object}.
Take 50K samples from this distribution as a train set, but apply the following
label noise: flip the label of cats to \texttt{Object} with probability 30\%.
Now train a WideResNet to 0 train error on this train set.
\end{experiment}

How do we expect the outputs of the trained classifier to behave on test samples?
Several options are: 
\begin{enumerate}
\item The classifier correctly classifies most cats as animals.
After all, there is only 3\% label noise in the overall train set, and we may expect that this is small enough that the network learns the right concept of \texttt{Animal} vs \texttt{Object} 

\item The label noise is ``spread'' across the animal class,
and all sub-classes (cat, dog, horse, deer, frog) have moderate misclassification errors at test time.
After all, the classifier is not explicitly told what a cat or a dog is, just that they are all animals.

\item The classifier misclassifies roughly 30\% of test cats as \texttt{Object},
but all other types of animals are largely unaffected.
\end{enumerate}

In fact, reality is closest to option (3).
The left panel in Figure \ref{fig:intro} shows the results of this experiment with a WideResNet-28-10 \citep{zagoruyko2016wide}.
The top panel shows the joint density of train inputs $x$ with train labels \texttt{Object/Animal}.
The bottom panel shows the joint density of test inputs $x$ with classifier predictions $f(x)$,
on the test set.
These joint densities are close.
In particular, although the classifier was not explicitly given
the labels of each type of animal, its errors were ``localized'' to the cat class -- reflecting
the same distribution as the train set. We discuss this ``locality'' further below. 



\begin{figure}[t]
    \centering
      \includegraphics[width=\textwidth]{figures/intro_supercat_illus_cm.png}
    \caption{
    {\bf Distributional Generalization in Experiment 1.}~~
    {\bf (A):}
    The CIFAR-10 train set is labeled as either \texttt{Animal/Object}, with label noise affecting only cats.
    A WideResNet-28-10 is then trained to 0 train error on this train set.
    The top panel shows the joint density of the train set: $(\texttt{CIFAR\_Class}(x), y)$.
    The bottom panels shows the joint density of classifier predictions on the test set:
    $(\texttt{CIFAR\_Class}(x), f(x))$.
    Distributional Generalization claims that these two joint densities are close.
    {\bf (B):} Simplified schematic showing that 1-nearest neighbors would reproduce this behavior.
    Dots indicate train points, colored by their train label \texttt{Animal/Object}.
    30\% of the cats in the train set are mislabeled as \texttt{Object},
    and we see that the 1-nearest neighbor decision boundary (shaded red/blue) mislabels roughly $30\%$ of the cat region as \texttt{Object}
    as well.
    That is, nearest-neighbor in an appropriate space would have similar behavior as we observe with WideResNets.
    }
    \label{fig:intro}
\end{figure}


Similarly, consider the following extension of this experiment.
\begin{experiment}
\label{exp:intro2}
Consider the following distribution over images $x$ and binary labels $y$.
Sample $x$ as a uniformly random CIFAR-10 image,
and sample the label as $p(y | x) = \textrm{Bernoulli}(\texttt{CIFAR\_Class(x)}/10)$.
That is, if the CIFAR-10 class of $x$ is $k \in \{0, 1, \dots 9\}$,
then the label is $1$ with probability $(k/10)$ and $0$ otherwise. 
Figure~\ref{fig:bnry-inc-wrn} shows this joint distribution of $(x, y)$.
As before, train a WideResNet to 0 training error on this distribution.
\end{experiment}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/Intro_Bin-Inc.png}
    \caption{{\bf Distributional Generalization in Experiment~\ref{exp:intro2}.}~~
    Joint densities of the distributions involved in Experiment \ref{exp:intro2}.
    The top panel shows the joint density of labels on the train set: $(\texttt{CIFAR\_Class(x)}, y)$.
    The bottom panels shows the joint density of classifier predictions on the test set: $(\texttt{CIFAR\_Class(x)}, f(x))$.
    Distributional Generalization claims that these two joint densities are close.
    }
    \label{fig:bnry-inc-wrn}
\end{figure}


Recall that we are using a method designed for classification,
and we hope to approximate the best-possible classifier.
In this setting, the Bayes-optimal classifier
(i.e. the classifier with minimal test error)
is the threshold function $f^*(x) = \1\{ \textrm{Class}(x) \geq 5 \}$,
which has 25\% test error.

However, a WideResNet trained to interpolation on this problem 
does \emph{not} behave like this optimal classifier -- it has $\approx 33\%$ test error.
When evaluated on the CIFAR-10 test set,
the network outputs label $1$ on roughly $(k/10)$ fraction of the examples in class $k$
--- the same distribution as the train set (as shown in Figure \ref{fig:bnry-inc-wrn}).
This example shows that the properties of classical generalization
and distributional generalization can be incompatible: in this case,
the best classically-generalizing classifier does not satisfy distributional generalization. Surprisingly, standard training procedures which were intended for classical generalization actually produce
a distributionally-generalizing classifier.

This example is also interesting because the network learnt to behave differently on each CIFAR-10 class (cat, dog, plane, etc),
even though it was not explicitly provided the CIFAR-10 labels.
This observation--- that powerful networks can pick up on
finer aspects of the distribution than their training labels reveal---
also exists in various forms in the literature.
For example, \citet{gilboa2019wider} found 
that standard CIFAR-10 networks
tend to cluster left-facing and right-facing horses separately
in activation space, when visualized via activation atlases~\citep{carter2019activation}.
Such fine-structural aspects of distributions can also be seen at the level of individual neurons (e.g. \citet{cammarata2020thread:,radford2017learning,olah2018building,zhou2014object,bau2020understanding}).




These behaviors are not captured by the classical framework of generalization, which only
discusses the test error of models.
Rather, they are better thought of as instances of the Indistinguishability Conjecture: the
train and test behaviors are close as distributions.

\subsection{Conjecture: Feature Calibration}
\label{intro:feat}

The distributional closeness of Experiments 1 and 2 is subtle,
and depends on the classifier architecture, distribution, and training method.
For example, Experiment \ref{exp:intro2} does not hold if we use a fully-connected network (MLP) instead of a ResNet,
or if we early-stop the ResNet instead of training to interpolation.
Both these scenarios fail in different ways:
An MLP cannot properly distinguish cats from dogs even when trained on real CIFAR-10 labels,
and so (informally) it has no hope of behaving differently on cats vs. dogs in the setting of Experiment \ref{exp:intro2} (See Fig. \ref{fig-app:bnry-inc-mlp} in Appendix \ref{app:density}).
On the other hand, an early-stopped ResNet for Experiment \ref{exp:intro2} does not label 30\% of cats as 1 on the \emph{train set},
since it does not interpolate, and thus has no hope of reproducing this behavior on the test set.
In fact, early-stopping training results in a classifier that is closer to Bayes-optimal,
but violates the distributional closeness of Experiment \ref{exp:intro2} (see Section~\ref{sec:gg}).

We characterize all of these behaviors, and their dependency on problem parameters,
via a formal conjecture.
Roughly, we claim that the output of interpolating classifiers 
is ``close'' to their input distribution, where this closeness is
``as good as we can hope'' given the power of the classifier.


\begin{boxedenv}{\bf Feature Calibration Conjecture (informal)}
{\it
``For interpolating classifiers $f$:
The distributions $(x, y)$ and $(x, f(x))$
on the test set look the same up to
features which can be distinguished by the architecture of $f$''
}
\end{boxedenv}

The formal version of this claim (Conjecture~\ref{conj:approx} in Section~\ref{sec:dist-features}),
can be seen as explicitly defining a
large family of tests $\mathcal{T}$ (the ``features which can be distinguished'')
for which the Indistinguishability Conjecture applies.
It captures behaviors far more general than Experiments 1 and 2,
and applies to neural networks, kernels, and decision trees.

    
    






\subsection{Conjecture: Agreement Property}
\label{intro:agree}
In Section~\ref{sec:agree} we present a seemingly unrelated set of experiments:
We observe that the test accuracy of a classifier is often close to
the probability that it agrees with an identically-trained classifier on a disjoint train set.

\begin{boxedenv}{\bf Agreement Conjecture (informal)}
{\it
``For two interpolating classifiers $f_1, f_2$
of the same architecture, trained on independent train sets from the same distribution $\cD$,
their \emph{agreement probability} on the test set
approximately matches their individual \emph{test accuracy}:
\begin{align}
\label{eqn:intro-aggr}
\Pr_{(x, y) \sim \cD}[ f_1(x) = f_2(x) ]
\approx
\Pr_{(x, y) \sim \cD}[ f_1(x) = y ]
\end{align}
}
\end{boxedenv}
For example, suppose we have two ResNets $f_1, f_2$
which were trained on independent train sets from the same distribution,
and both achieve test accuracy say 50\% on a 10-class problem.
That is, they agree with the true label $y(x)$ w.p 50\%.
Now we ask, what is the probability they
agree with \emph{each other}?
Depending on our intuition, we may expect:
(1) They agree with each other much less than they agree with the true label,
since each individual classifier is an independently noisy version of the truth.
(2) They agree with each other much more than 50\%, since
classifiers tend to have ``correlated'' predictions.

However, surprisingly, none of these are the case.
We show that for a variety of realistic domains and classifiers,
the agreement probability \emph{closely matches} the test accuracy.
In fact, this can be seen as an instance of the Indistinguishably Conjecture
for a specific test $\mathcal{T}$,
as we explain in Section~\ref{sec:agree}.

These experimental observations are independently interesting,
and could be useful for future applications.
For example, the LHS
of Equation~\ref{eqn:intro-aggr} is an estimate of the test error
that requires only unlabeled test examples $x$.



\subsection{Potential Mechanisms and Locality}

Throughout this work, we focus on formally characterizing
the observed behaviors (via our conjectures), and empirically testing
our conjectures in a variety of realistic settings.
However, we do not yet understand \emph{why} these conjectures hold across such a wide variety of domains.
One possible intuition for these behaviors is that interpolating classifiers
are (for some reason) behaving like \emph{local} estimators.

For example, note that 1-Nearest-Neighbors (in an appropriate metric space)
would reproduce the behavior we observe in Experiments 1 and 2.
To see this, consider a metric space in which the original CIFAR-10 classes are well-separated,
as shown schematically in Figure \ref{fig:intro}.
For a 1-Nearest-Neighbor (1-NN) classifier in this space,
the classifier outputs for test cats would match the distribution of training labels for cats.
In Experiment 2, for example, label noise that affects only cats in the train set would also
only affect cats at test time.
In this sense, the classifier behaves like a \emph{local} estimator.
While we do not make a formal connection between 1-NN and other interpolating classifiers,
many of the properties we discuss in this paper are shared between the two, and can be formally proved for 1-NN.
This is especially surprising for interpolating neural networks and kernel machines,
which are not usually considered ``local'' estimators.

We prove our conjectures for 1-Nearest-Neighbors in this work (Theorem~\ref{thm:Ltest}),
and we leave better understanding this potential connection as an important area for future work.

\subsection{Summary of Contributions}

We extend the classical framework of generalization
by introducing Distributional Generalization, in which
the train and test behavior of models are close \emph{as distributions}.
Informally, for a trained classifier $f$,
its outputs on the train set
$(x, f(x))_{x \in \TrainSet}$
are close in distribution to its outputs on the test set
$(x, f(x))_{x \in \TestSet}$,
where the form of this closeness depends on specifics of the model, training procedure, and distribution.

This notion is both more fine-grained than classical generalization -- in that it
considers the entire distribution of model outputs instead of a single functional --
as well as more robust:
even models which do not generalize well in the classical sense
can be well-behaved in a certain distributional sense.
In fact, for noisy distributions, distributional generalization 
is incompatible with classical generalization. And yet, we find
that standard methods in machine learning, which were intended to classically
generalize, actually distributionally generalize.



We initiate the study of Distributional Generalization
across various domains in machine learning, focusing primarily on interpolating classifiers.
For interpolating classifiers, we state two formal conjectures which predict the form of distributional closeness that can be expected for a given model and task:
\begin{enumerate}
    \item Feature Calibration Conjecture (Section~\ref{sec:dist-features}):
    Interpolating classifiers, when trained on samples from a distribution, 
    will match this distribution up to all ``distinguishable features'' (Definition~\ref{def:dist-feature-L}).
    \item Agreement Conjecture (Section~\ref{sec:agree}):
    For two interpolating classifiers of the same type,
    trained independently on the same distribution,
    their \emph{agreement probability} with each other on test samples
    roughly matches their \emph{test accuracy}.
\end{enumerate}

We perform a number of experiments surrounding these conjectures.
These experiments reveal new behaviors of standard interpolating classifiers
(e.g. ResNets, MLPs, kernels, decision trees), and are independently interesting.
Finally, we discuss extending these results to non-interpolating methods in Section~\ref{sec:gg},
and we give preliminary evidence for a third form of distributional closeness in Appendix~\ref{sec:student}.


    
    





==> sec_Ltest.tex <==
\section{Feature Calibration}
\label{sec:dist-features}

In this section, we present our first formal conjecture
which characterizes a family of tests $\mathcal{T}$ for which the output distribution of a classifier $(x, f(x)) \sim \Dte$
is ``close'' to the source distribution $(x, y) \sim \cD$.
This family of tests is subtle to define,
because we cannot expect closeness in total variation distance (which corresponds to closeness in all possible bounded functions).
Rather, the best we can hope for (informally) is that the classifier's output
matches the true distribution along all features that it can learn.
At a high level, we will argue that the distributions $\Dte$ and $\cD$
are statistically close if we first ``coarsen'' the domain of $x$ by some
labelling $L: \cX \to [M]$. 
That is, for certain partitions $L$, the following
distributions are statistically close:
\begin{align*}
(L(x), f(x)) &\approx_{\eps} (L(x), y)
\end{align*}



We first explain this conjecture (``Feature Calibration'') via a toy example, and then we formalize it in Section~\ref{sec:formal}.

\subsection{Toy Example}
\label{sec:toy}
\newcommand{\fpart}[1]{\hyperref[fig:partition]{\ref*{fig:partition}#1}}




Consider a distribution on points $x \in \R^2$ and binary labels $y$, as visualized in
Figure~\fpart{A}.
This distribution consists of four clusters 
\texttt{\{Truck, Ship, Cat, Dog\}} which are labeled either
\texttt{Object} or \texttt{Animal}, depicted in red and blue respectively.
One of these clusters --- the \texttt{Cat} cluster --- is mislabeled as class \texttt{Object} with probability 30\%.
Now suppose we have an interpolating classifier $f$ for this distribution, obtained in some way,
and wish to quantify the closeness between distributions $(x, y) \approx (x, f(x))$ on the test set.
Figure~\fpart{A} shows test points $x$ along with their test labels $y$ -- these
are samples from the source distribution $\cD$.
Figure~\fpart{B} shows these same test points, but labeled according to $f(x)$ --
these are samples from the test distribution $\Dte$.
The shaded red/blue regions in Figure~\fpart{B} shows the decision boundary of the classifier $f$.

These two distributions do not match exactly -- there are some test points where the true label $y$ and classifier output $f(x)$ disagree.
However, if we ``coarsen'' the domain into the four clusters \texttt{\{Truck, Ship, Cat, Dog\}},
then the marginal distribution of labels within each cluster matches between the classifier outputs $f(x)$
and true labels $y$.
In particular, the fraction of \texttt{Cat} points that are labeled \texttt{Object} is similar between
Figures~\fpart{C} and \fpart{D}.
This is equivalent to saying that the joint distributions $(L(x), y)$ and $(L(x), f(x))$ 
are statistically close, for the partition $L: \cX \to \texttt{\{Truck, Ship, Cat, Dog\}}$.
That is, if we can only see points $x$ through their cluster-label $L(x)$,
then the distributions $(x, y)$ and $(x, f(x))$ will appear close.
These two ``coarsened'' joint distributions are also what we plotted in Figure~\ref{fig:intro}
from the Introduction, where we considered the partition $L(x) := \texttt{CIFAR\_Class}(x)$, the CIFAR-10 class of $x$.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/L-test-illus.png}
\caption{{\bf Toy Example: Feature Calibration.}
Schematic of the distributions discussed in Section~\ref{sec:toy},
showing a toy example of the Feature Calibration conjecture for several distinguishable features $L$.
}
\label{fig:partition}
\end{figure}

There may be many such partitions $L$ for which the above distributional closeness holds.
For example, the coarser partition $L_2: \cX \to \texttt{\{Animal, Object\}}$ also
works in our example, as shown in Figures~\fpart{E} and \fpart{F}.
However, clearly not all partitions $L$ will satisfy closeness, since the distributions themselves
are not statistically close. 
For a finer partition which splits the clusters into smaller pieces (e.g. based on the age of the dog),
the distributions may not match unless we use very powerful classifiers or many train samples.
To formalize the set of allowable partitions $L$,
we define a \emph{distinguishable feature}:
a partition of the domain $\cX$ that is learnable for a given family of models. 
Intuitively, both of the partitions considered above are reasonable, because they can be
\emph{learnt} from samples.

\subsection{Formal Definitions}
\label{sec:formal}
Here we define a \emph{distinguishable feature}:
a labeling of the domain $\cX$ that is learnable for a given family of models. 
This definition depends on the family of models $\cF$, the distribution $\cD$,
and the number of train samples $n$.
\begin{definition}[$(\eps, \cF, \cD, n)$-Distinguishable Feature]
\label{def:dist-feature-L}
For a distribution $\cD$ over $\cX \x \cY$,
number of samples $n$,
family of models $\cF$, and small $\eps \geq 0$,
an \emph{$(\eps, \cF, \cD, n)$-distinguishable feature}
is a partition $L: \cX \to [M]$
of the domain $\cX$ into $M$ parts, such that
training a model from $\cF$
on $n$ samples labeled by $L$
works to classify $L$ with high test accuracy.

Precisely, $L$ is a distinguishable feature if the following procedure succeeds with probability at least $1-\eps$:
\begin{enumerate}
    \item Sample a train set $S \gets \{(x_i, L(x_i))\}$ of $n$ samples $(x_i, y_i) \sim \cD$,
    labeled by the partition $L$.
    \item Train a classifier $f \gets Train_{\cF}(S)$.
    \item Sample a test point $x \sim \cD$, and check that $f$ correctly classifies its partition:
    Output success iff $f(x) = L(x)$.
\end{enumerate}
That is, $L$ is a $\epsL$-distinguishable feature if:
$$
\Pr_{\substack{
S = \{(x_i, L(x_i)\}_{x_1, \dots, x_n \sim \cD}\\
f \gets \Train_{\cF}(S)\\
x \sim \cD
}}[
f(x) = L(x)
]
\geq 1-\eps
$$
\end{definition}
To recap, this definition is meant to
capture a labeling of the domain $\cX$ that is learnable for a given family of models and training procedure.
For example, in Experiment~\ref{exp:intro1}, the CIFAR-10 class partition
$L(x) := \textrm{Class}(x)$ is a distinguishable feature for ResNets trained with Stochastic Gradient Descent given 50k samples,
since ResNets are capable of learning this labeling from samples.
Note that this definition only depends on the marginal distribution of $\cD$ on $x$,
and does not depend on the label distribution $p_{\cD}(y | x)$.

The definition of distinguishable feature must depend on the classifier family $\cF$ and number of samples $n$,
since a more powerful classifier can distinguish more features.
For example, the CIFAR-10 classes are \emph{not} a
distinguishable feature for MLPs.
This distinction is important ---
if we run the same Experiment~\ref{exp:intro1} in the Introduction with an
MLP instead of a ResNet, the MLP will not match the distribution $\cD$ nearly as closely (See Appendix \ref{app:density}).
Intuitively, the ResNet was able to act differently on cats compared to dogs
at test time because it can distinguish these classes of CIFAR-10.
However, the MLP will not be able to act
very differently on cats vs. dogs, because it cannot distinguish these classes as
accurately.
Note that there could be many distinguishable features for a given setting $\epsL$ ---
including features not implied by the class label
such as the presence of grass in a CIFAR-10 image. 




Our main conjecture in this section is that
the test distribution $(x, f(x)) \sim \Dte$
is statistically close to the source distribution $(x, y) \sim \cD$
when the domain is ``coarsened'' by a distinguishable feature.
That is, the distributions $(L(x), f(x))$ and $(L(x), y)$
are \emph{statistically} close for all distinguishable features $L$.
Formally:




\begin{conjecture}[Feature Calibration]
\label{conj:approx}
For all natural distributions $\cD$,
number of samples $n$,
family of interpolating models $\cF$,
and $\eps \geq 0$,
the following distributions are statistically close for all $\epsL$-distinguishable features $L$:
\begin{align}
\underset{
\substack{
f \gets \Train_{\cF}(\cD^n)\\
x, y \sim \cD
}
}{
(L(x), f(x))
}
\quad\approx_\eps\quad
\underset{
x, y \sim \cD
}{
(L(x), y)
}
\end{align}
\end{conjecture}






Notably, this holds \emph{for all} distinguishable features $L$,
and it holds ``automatically'' -- we simply train a classifier, without specifying any particular partition.
The statistical closeness predicted is within $\eps$, which is determined by the $\eps$-distinguishability
of $L$ (we usually think of $\eps$ as small).
As a trivial instance of the conjecture,
suppose we have a distribution with deterministic labels,
and consider the $\eps$-distinguishable feature $L(x) := y(x)$, i.e. the label itself.
The $\eps$ here is then simply the test error of $f$,
and Conjecture~\ref{conj:approx} is true by definition.

The formal statements of Definition~\ref{def:dist-feature-L} and Conjecture~\ref{conj:approx}
may seem somewhat arbitrary, involving many quantifiers over $\epsL$.
However, we believe these statements are natural.
To support this, in Section~\ref{sec:1nn} we prove that Conjecture~\ref{conj:approx} is formally
true as stated for 1-Nearest-Neighbor classifiers.

{\bf Connection to Indistinguishability.}
Conjecture~\ref{conj:approx} can be equivalently phrased as an instantiation of our general
Indistinguishably Conjecture:
the source distribution $\cD$ and 
test distribution $\Dte$ are
``indistinguishable up to $L$-tests''.
That is, Conjecture~\ref{conj:approx}
is equivalent to the statement 
\begin{align}
\Dte \approx_\eps^{\cL} \cD
\end{align}
where $\cL$ is the family of all tests which depend on $x$
only via a distinguishable feature $L$. That is,
$
\cL := \{(x, y) \mapsto T(L(x), y) :
(\eps, \cF, \cD, n)\text{-distinguishable feature }L
\text{ and } T: [M] \x \cY \to [0, 1] \}
$. In other words, $\Dte$ is indistinguishable from $\cD$
to any distinguisher that only sees the input $x$ via a distinguishable feature $L(x)$.






\subsection{Experiments}
We now empirically validate our conjecture in a variety of settings in machine learning,
including neural networks, kernel machines, and decision trees.
To do so, we begin by considering the simplest possible distinguishable feature,
and progressively consider more complex ones. 
Each of the experimental settings below highlights a different aspect of interpolating classifiers,
which may be of independent theoretical or practical interest.
We summarize the experiments here; detailed descriptions are provided in Appendix~\ref{app:density}.

\textbf{Constant Partition:} Consider the trivially-distinguishable \emph{constant} feature $L(x) = 0$.
Then, Conjecture~\ref{conj:approx} states that the marginal distribution
of class labels for any interpolating classifier $f(x)$
is close to the true marginals $p(y)$.
That is, irrespective of the classifier's test accuracy, it outputs the ``right'' proportion of class labels on the test set, even when there is strong class imbalance.

To show this, we construct a dataset based on CIFAR-10 that has class imbalance. For class $k \in \{0...9\}$, sample $(k+1)\times 500$ images from that class. This will give us a dataset where classes will have marginal distribution $p(y = \ell) \propto \ell+1$ for classes $\ell \in [10]$, as shown in Figure \ref{fig:constant-L}. We do this both for the training set and the test set, to keep the distribution $\cD$ fixed.


We then train a variety of classifiers (MLPs, Kernels, ResNets) to interpolation on this dataset,
which have varying levels of test errors (9-41\%).
The class balance of classifier outputs on the (rebalanced) test set
is then close to the class balance on the train set, even for poorly generalizing classifier. Full experimental details and results are described in Appendix \ref{app:density}.
Note that a 1-nearest neighbors classifier would have this property.

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/constant_L.png}
    \centering
    \caption{{\bf Feature Calibration for Constant Partition $L$: }
     The CIFAR-10 train and test sets are class rebalanced according to (A).
     Interpolating classifiers are trained on the train set,
     and we plot the class balance of their outputs on the test set.
     This roughly matches the class balance of the train set, even for poorly-generalizing classifiers.}
    \label{fig:constant-L}
\end{figure}









{\bf Class Partition:} We now consider settings (datasets and models)
where the original class labels are a distinguishable feature.
For instance, the CIFAR-10 classes are distinguishable by ResNets,
and MNIST classes are distinguishable by the RBF kernel. Since the conjecture holds for any arbitrary label distribution $p(y|x)$, we consider many such label distributions and show that, for instance, the joint distributions $(\textrm{Class}(x), y)$ and $(\textrm{Class}(x), f(x))$ are close. This includes the setting of Experiments 1 and 2 from the Introduction. 

\begin{figure}[p]
    \includegraphics[width=\linewidth]{figures/cifar10_wrn_target_varyp.png}
    \centering
    \caption{\textbf{Feature Calibration with original classes on CIFAR-10}: We train a WRN-28-10 on the CIFAR-10 dataset where we mislabel class $0 \rightarrow 1$ with probability $p$.
    (A): Joint density of the distinguishable features $L$ (the original CIFAR-10 class) and the classification task labels $y$ on the train set for noise probability $p=0.4$.
    (B): Joint density of the original CIFAR-10 classes $L$ and the network outputs $f(x)$ on the test set.
    (C): Observed noise probability in the network outputs on the test set (the (1, 0) entry of the matrix in B) for varying noise probabilities $p$}
    \label{fig:target-varyp}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[width=0.7\linewidth]{figures/WRN_randomv4.png}
\caption{{\bf Feature Calibration with random confusion matrix on CIFAR-10: }
Left: Joint density of labels $y$ and original class $L$ on the train set.
Right: Joint density of classifier predictions $f(x)$ and original class $L$
on the test set,
for a WideResNet28-10 trained to interpolation. These two joint densities are close,
as predicted by Conjecture~\ref{conj:approx}.}
\label{fig:wrn_random}
\end{figure}

\begin{figure}[p]
    \includegraphics[width=\linewidth]{figures/molbio.png}
    \centering
    \caption{{\bf Feature Calibration for Decision trees on UCI (molecular biology).}
    We add label noise that takes class $2$ to class $1$ with probability $p \in [0, 0.5]$.
    The top row shows the confusion matrix of the true class $L(x)$ vs. the label $y$
    on the train set, for varying levels of noise $p$.
    The bottom row shows the corresponding confusion matrices of the classifier predictions $f(x)$
    on the test set, which closely matches the train set, as predicted by Conjecture~\ref{conj:approx}.
    }
    \label{fig:dtdna}
\end{figure}


In Figure \ref{fig:target-varyp}, we mislabel class $0 \rightarrow 1$ with probability $p$ in the CIFAR-10 train set. This gives us the joint distribution shown in Figure \ref{fig:target-varyp}A. 
We then train a WideResNet-28-10 (WRN-28-10) on this noisy distribution.
Figure \ref{fig:target-varyp}B shows the joint distribution on the test set.
Figure \ref{fig:target-varyp}C shows the $(1, 0)$ entry of this matrix as we vary $p \in [0, 1]$.
The Bayes optimal classifier for this distribution would behave as a step function (shown in red),
and a classifier that obeys Conjecture 1 exactly would follow the diagonal (in green).
The actual experiment (in blue) is close to the behavior predicted by Conjecture 1.




In fact, we conjecture holds even for a random joint density matrix on CIFAR-10.
In Figure~\ref{fig:wrn_random}, we first generate a random sparse
confusion matrix on 10 classes, such that each class is preserved with probability 50\%
and flipped to one of two other classes with probability 20\% and 30\% respectively.
We then apply label noise with this confusion matrix to the train set,
and measure the confusion matrix of the trained classifier on the test set.
As expected, the train and test confusion matrices are close, and share the same sparsity pattern.




Figure~\ref{fig:dtdna} shows a version of this experiment for decision trees on
the molecular biology UCI task.
The molecular biology task is a 3-way classification problem: to classify the type of 
a DNA splice junction (donor, acceptor, or neither), given the sequence of DNA (60 bases) surrounding the junction.
We add varying amounts of label noise that flips class 2 to class 1
with a certain probability, and we observe that interpolating decision trees reproduce
this same structured label noise on the test set.
We also demonstrate similar experiments with the Gaussian kernel on MNIST (Figure \ref{fig:kernelgg}),
and several other UCI tasks (Appendix~\ref{app:density}).



{\bf Multiple features:} We now consider a setting where we may have many distinguishable features for a single classification task. The conjecture states that the network should be automatically calibrated for all distinguishable features, even when it is not explicitly provided any information about these features.  For this, we use the CelebA dataset~\citep{liu2015faceattributes},
which contains images of celebrities with various labelled binary attributes per-image (``male'', ``blond hair'', etc). Some of these attributes form a distinguishable feature for ResNet50 as they are learnable to high accuracy \citep{jahandideh2018physical}. We pick one of the hard attributes as the target classification task, where a ResNet-50 achieves 80\% accuracy.  Then we confirm that the output distribution is calibrated with respect to the attributes that form distinguishable features. In this setting, the label distribution is deterministic, and not directly dependent on the distinguishable features, unlike the experiments considered before. Yet, as we see in Figure~\ref{fig:celeba_wrap}, the classifier outputs are correctly calibrated for each attribute. Full details of the experiment are described in Appendix \ref{app:celeba}.


\begin{figure}
\centering
\includegraphics[width=0.6\linewidth]{figures/CelebAv2.png}
\caption{\textbf{Feature Calibration for multiple features on CelebA}: We train a ResNet-50 to perform binary classification task on the CelebA dataset. The top row shows the joint distribution of this task label with various other attributes in the dataset. The bottom row shows the same joint distribution for the ResNet-50 outputs on the test set. Note that the network was not given any explicit inputs about these attributes during training.}
\label{fig:celeba_wrap}
\end{figure}




\textbf{Coarse Partition:}
Consider AlexNet trained on ImageNet ILSVRC-2012 \citep{ILSVRC15},
a 1000-class image classification problem including 116 varieties of dogs.
The network only achieves 56.5\% accuracy on the test set, but
it has higher accuracy on coarser label partitions:
for example, it will at least classify most dogs as dogs (with 98.4\% accuracy), though it may mistake the specific dog variety.
In this example, $L(x) \in \{\text{dog, not-dog}\}$ is the distinguishable feature.
Moreover, the network is \emph{calibrated} with respect to dogs:
22.4\% of all dogs in ImageNet are Terriers,
and indeed, the network classifies 20.9\% of all dogs as Terriers
(though it has 9\% error in which specific dogs it classifies as Terriers).
We include similar experiments with ResNets and kernels in Appendix~\ref{app:density}.

\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
Model &  AlexNet &  ResNet50 \\
\midrule
ImageNet accuracy                            &    {\bf 0.565} &     0.761 \\
Accuracy on terriers                         &    0.572 &     0.775 \\
Accuracy for binary \{dog/not-dog\}            &    0.984 &     0.996 \\
Accuracy on \{terrier/not-terrier\} among dogs &    0.913 &     0.969 \\
\midrule
Fraction of real-terriers among dogs         &    {\bf 0.224} &     0.224 \\
Fraction of predicted-terriers among dogs    &    {\bf 0.209} &     0.229 \\
\bottomrule
\end{tabular}
\caption{{\bf Feature Calibration on ImageNet: }
ImageNet classifiers are calibrated with respect to dogs.
For example, all classifiers predict terrier for roughly $\sim22\%$ of all dogs (last row),
though they may mistake which specific dogs are terriers.
See Table~\ref{tab:imagenet} in the Appendix for more models.}
\label{tab:imagenet-trunc}
\end{table}










\subsection{Discussion}
Conjecture~\ref{conj:approx} claims that $\Dte$
is close to $\cD$ up to all tests which are
\emph{themselves learnable}.
That is, if an interpolating method
is capable of learning a certain partition of the domain,
then it will also produce outputs that are calibrated
with respect to this partition, when trained on any problem.
This conjecture thus gives a way of quantifying the resolution
with which classifiers approximate the source distribution $\cD$, 
via properties of the classification algorithm itself.
This is in contrast to many classical ways of
quantifying the approximation of density estimators,
which rely on \emph{analytic} (rather than \emph{operational})
distributional assumptions~\citep{tsybakov2008introduction, wasserman2006all}.

{\bf Proper Scoring Rules.}
If the loss function used in training is a \emph{strictly-proper scoring rule}
such as cross-entropy~\citep{gneiting2007strictly},
then we may expect that in the limit of a large-capacity network
and infinite data, training on samples $\{(x_i, y_i)\}$
will yield a good density estimate of $p(y | x)$ at the softmax layer.
However, this is not what is happening in our experiments:
First, our experiments consider the hard-decisions, not the softmax outputs.
Second, we observe Conjecture~\ref{conj:approx}
even in settings without proper scoring rules
(e.g. kernel SVM and decision trees).


\subsection{1-Nearest-Neighbors Connection}
\label{sec:1nn}
Here we show that the 1-nearest neighbor classifier provably satisfies
Conjecture~\ref{conj:approx}, under mild assumptions.
This is trivially true when the number of train points $n \to \infty$,
such that the train points pack the domain.
However, we do not require any such assumptions:
the theorem below applies generically to a wide class of distributions,
with no assumptions on the ambient dimension of inputs,
the underlying metric, or smoothness of the source distribution.
All the distributional requirements are captured by the preconditions of
Conjecture~\ref{conj:approx}, which require that the feature $L$
is $\eps$-distinguishable to 1-Nearest-Neighbors.
The only further assumption is a weak regularity condition:
sampling the nearest neighbor train point to a random test point
should yield (close to) a uniformly random test point.
In the following, $\NN_S(x)$ refers to the nearest neighbor of point $x$ among points in set $S$.

\begin{theorem}
\label{thm:Ltest}
Let $\cD$ be a distribution over $\cX \x \cY$, and let $n \in \N$ be the number of train samples.
Assume the following regularity condition holds:
Sampling the nearest neighbor train point to a random test point
yields (close to) a uniformly random test point.
That is, suppose that for some small $\delta \geq 0$,
\begin{align}
\{\NN_S(x)\}_{\substack{
S \sim \cD^n\\
x \sim \cD
}}
\quad\approx_\delta\quad
\{x\}_{\substack{
x \sim \cD
}}
\end{align}
Then, Conjecture~\ref{conj:approx} holds. For all $(\eps, \NN, \cD, n)$-distinguishable partitions $L$,
the following distributions are statistically close:
\begin{align}
\{(y, L(x))\}_{x, y \sim \cD}
\quad\approx_{\eps + \delta}\quad
\{(\NNf_S(x), L(x)\}_{\substack{
S \sim \cD^n\\
x, y \sim \cD
}}
\end{align}
\end{theorem}
The proof of Theorem~\ref{thm:Ltest} is straightforward, and provided in Appendix~\ref{sec:proofs}.
We view this theorem both as support for our formalism of Conjecture~\ref{conj:approx},
and as evidence that the classifiers we consider in this work have \emph{local} properties
similar to 1-Nearest-Neighbors.

Note that Theorem~\ref{thm:Ltest} does not hold for the k-nearest neighbor classifier (k-NN),
which takes the plurality vote of K neighboring train points.
However, it is somewhat more general than 1-NN: for example, it holds for a randomized version of K-NN which,
instead of taking the plurality,
randomly picks one of the K neighboring train points (potentially weighted) for the test classification.


\subsection{Pointwise Density Estimation}
\label{sec:ptwise}
In fact, we could hope for an even stronger property than
Conjecture~\ref{conj:approx}.
Consider the familiar example:
we mislabel 20\% of dogs as cats in the CIFAR-10 training data,
and train an interpolating ResNet on this train set.
Conjecture~\ref{conj:approx} predicts that, \emph{on average}
over all test dogs, roughly 20\% of them are classified as cats.
In fact, we may expect this to hold pointwise for each dog:
For a single test dog $x$, if we train a new classifier $f$ (on fresh iid samples from the noisy distribution),
then $f(x)$ will be cat roughly 20\% of the time.
That is, for each test point $x$, taking an ensemble over independent train sets yields an estimate of the conditional density $p(y | x)$.
Informally:
\begin{align}
\text{With high probability over test } x \sim \cD:
\quad
\Pr_{f \gets \Train_{\cF}(\cD^n)}[f(x) = \ell] ~\approx~ p(y = \ell | x)
\end{align}
where the probability on the LHS is over the random sampling of train set, and any randomness in the training procedure.
This behavior would be stronger than,
and not implied by, Conjecture~\ref{conj:approx}.
We give preliminary experiments supporting such a pointwise property in Appendix~\ref{app:ptwise}.



==> sec_blank.tex <==

\section{test}
Placeholder.
\newpage

==> sec_broader.tex <==
\section{Broader Impact}
Our paper aims to deepen our theoretical understanding of a broad range of supervised classification methods. Many of these classifiers, for instance deep neural networks, are poorly understood and are often treated as black-box classifiers. We hope that our work will contribute to demystifying these methods, some of which are already being deployed widely.%


==> uci_results.tex <==
\begin{tabular}{lllllll} 
\toprule \\ 
Name & $n$ & $d$    & Classes & Test Acc. F1 ( mean )    & Test Acc. F2 ( mean ) & Agreement Probability ( mean ) \\ 
\midrule \\ 
\verb!abalone! & 4177 & 8 & 3 & 0.55 (0.55) & 0.56 (0.55) & 0.56 (0.54)\\ 
\verb!acute-inflammation! & 120 & 6 & 2 & 1.00 (0.96) & 1.00 (0.95) & 1.00 (0.92)\\ 
\verb!acute-nephritis! & 120 & 6 & 2 & 1.00 (0.97) & 1.00 (0.97) & 1.00 (0.96)\\ 
\verb!adult! & 48842 & 14 & 2 & 0.80 (0.81) & 0.81 (0.81) & 0.80 (0.80)\\ 
\verb!annealing! & 898 & 31 & 5 & 0.88 (0.88) & 0.92 (0.87) & 0.82 (0.83)\\ 
\verb!arrhythmia! & 452 & 262 & 13 & 0.43 (0.50) & 0.58 (0.49) & 0.47 (0.43)\\ 
\verb!audiology-std! & 196 & 59 & 18 & 0.38 (0.50) & 0.55 (0.51) & 0.38 (0.38)\\ 
\verb!balance-scale! & 625 & 4 & 3 & 0.73 (0.75) & 0.75 (0.75) & 0.74 (0.69)\\ 
\verb!balloons! & 16 & 4 & 2 & 0.50 (0.54) & 1.00 (0.59) & 0.50 (0.53)\\ 
\verb!bank! & 4521 & 16 & 2 & 0.84 (0.85) & 0.81 (0.85) & 0.81 (0.84)\\ 
\verb!blood! & 748 & 4 & 2 & 0.73 (0.71) & 0.70 (0.71) & 0.78 (0.73)\\ 
\verb!breast-cancer! & 286 & 9 & 2 & 0.64 (0.63) & 0.66 (0.63) & 0.67 (0.63)\\ 
\verb!breast-cancer-wisc! & 699 & 9 & 2 & 0.94 (0.93) & 0.94 (0.93) & 0.94 (0.93)\\ 
\verb!breast-cancer-wisc-diag! & 569 & 30 & 2 & 0.93 (0.91) & 0.86 (0.91) & 0.90 (0.89)\\ 
\verb!breast-cancer-wisc-prog! & 198 & 33 & 2 & 0.72 (0.65) & 0.80 (0.65) & 0.68 (0.62)\\ 
\verb!breast-tissue! & 106 & 9 & 6 & 0.55 (0.52) & 0.45 (0.53) & 0.36 (0.46)\\ 
\verb!car! & 1728 & 6 & 4 & 0.86 (0.87) & 0.86 (0.87) & 0.78 (0.81)\\ 
\verb!cardiotocography-10clases! & 2126 & 21 & 10 & 0.64 (0.67) & 0.66 (0.68) & 0.55 (0.59)\\ 
\verb!cardiotocography-3clases! & 2126 & 21 & 3 & 0.86 (0.87) & 0.87 (0.88) & 0.83 (0.84)\\ 
\verb!chess-krvk! & 28056 & 6 & 18 & 0.52 (0.53) & 0.54 (0.53) & 0.40 (0.40)\\ 
\verb!chess-krvkp! & 3196 & 36 & 2 & 0.94 (0.92) & 0.95 (0.92) & 0.91 (0.88)\\ 
\verb!congressional-voting! & 435 & 16 & 2 & 0.61 (0.59) & 0.56 (0.58) & 0.26 (0.59)\\ 
\verb!conn-bench-sonar-mines-rocks! & 208 & 60 & 2 & 0.79 (0.67) & 0.71 (0.66) & 0.74 (0.62)\\ 
\verb!conn-bench-vowel-deterding! & 990 & 11 & 11 & 0.63 (0.68) & 0.61 (0.68) & 0.47 (0.52)\\ 
\verb!connect-4! & 67557 & 42 & 2 & 0.76 (0.77) & 0.77 (0.77) & 0.72 (0.72)\\ 
\verb!contrac! & 1473 & 9 & 3 & 0.51 (0.46) & 0.47 (0.46) & 0.47 (0.44)\\ 
\verb!credit-approval! & 690 & 15 & 2 & 0.78 (0.75) & 0.83 (0.75) & 0.72 (0.70)\\ 
\verb!cylinder-bands! & 512 & 35 & 2 & 0.61 (0.64) & 0.64 (0.63) & 0.50 (0.59)\\ 
\verb!dermatology! & 366 & 34 & 6 & 0.70 (0.82) & 0.78 (0.83) & 0.57 (0.75)\\ 
\verb!echocardiogram! & 131 & 10 & 2 & 0.63 (0.75) & 0.70 (0.74) & 0.63 (0.72)\\ 
\verb!ecoli! & 336 & 7 & 8 & 0.68 (0.70) & 0.69 (0.71) & 0.63 (0.64)\\ 
\verb!energy-y1! & 768 & 8 & 3 & 0.94 (0.90) & 0.94 (0.90) & 0.88 (0.86)\\ 
\verb!energy-y2! & 768 & 8 & 3 & 0.89 (0.89) & 0.91 (0.88) & 0.89 (0.87)\\ 
\verb!fertility! & 100 & 9 & 2 & 0.85 (0.79) & 0.70 (0.79) & 0.85 (0.80)\\ 
\verb!flags! & 194 & 28 & 8 & 0.47 (0.40) & 0.55 (0.40) & 0.55 (0.32)\\ 
\verb!glass! & 214 & 9 & 6 & 0.52 (0.58) & 0.57 (0.58) & 0.39 (0.51)\\ 
\verb!haberman-survival! & 306 & 3 & 2 & 0.61 (0.65) & 0.69 (0.66) & 0.56 (0.66)\\ 
\verb!hayes-roth! & 160 & 3 & 3 & 0.59 (0.67) & 0.59 (0.67) & 0.44 (0.60)\\ 
\verb!heart-cleveland! & 303 & 13 & 5 & 0.44 (0.47) & 0.34 (0.47) & 0.44 (0.43)\\ 
\verb!heart-hungarian! & 294 & 12 & 2 & 0.68 (0.75) & 0.73 (0.74) & 0.75 (0.73)\\ 
\verb!heart-switzerland! & 123 & 12 & 5 & 0.28 (0.32) & 0.28 (0.32) & 0.20 (0.30)\\ 
\verb!heart-va! & 200 & 12 & 5 & 0.23 (0.28) & 0.28 (0.29) & 0.30 (0.25)\\ 
\verb!hepatitis! & 155 & 19 & 2 & 0.71 (0.76) & 0.87 (0.77) & 0.71 (0.75)\\ 
\verb!hill-valley! & 1212 & 100 & 2 & 0.55 (0.50) & 0.49 (0.51) & 0.50 (0.50)\\ 
\verb!horse-colic! & 368 & 25 & 2 & 0.68 (0.72) & 0.80 (0.73) & 0.69 (0.69)\\ 
\verb!ilpd-indian-liver! & 583 & 9 & 2 & 0.67 (0.65) & 0.69 (0.65) & 0.65 (0.64)\\ 
\verb!image-segmentation! & 2310 & 18 & 7 & 0.88 (0.90) & 0.91 (0.90) & 0.84 (0.87)\\ 
\verb!ionosphere! & 351 & 33 & 2 & 0.76 (0.81) & 0.77 (0.82) & 0.70 (0.76)\\ 
\verb!iris! & 150 & 4 & 3 & 0.93 (0.93) & 0.93 (0.93) & 0.93 (0.92)\\ 
\verb!led-display! & 1000 & 7 & 10 & 0.68 (0.67) & 0.67 (0.67) & 0.73 (0.75)\\ 
\verb!lenses! & 24 & 4 & 3 & 0.50 (0.61) & 0.67 (0.66) & 0.67 (0.52)\\ 
\verb!letter! & 20000 & 16 & 26 & 0.76 (0.76) & 0.77 (0.76) & 0.68 (0.66)\\ 
\verb!libras! & 360 & 90 & 15 & 0.44 (0.42) & 0.42 (0.40) & 0.26 (0.24)\\ 
\verb!low-res-spect! & 531 & 100 & 9 & 0.80 (0.79) & 0.80 (0.80) & 0.76 (0.76)\\ 
\verb!lung-cancer! & 32 & 56 & 3 & 0.25 (0.38) & 0.38 (0.40) & 0.25 (0.34)\\ 
\verb!lymphography! & 148 & 18 & 4 & 0.57 (0.72) & 0.73 (0.69) & 0.50 (0.66)\\ 
\verb!magic! & 19020 & 10 & 2 & 0.78 (0.79) & 0.79 (0.79) & 0.75 (0.77)\\ 
\verb!mammographic! & 961 & 5 & 2 & 0.78 (0.76) & 0.70 (0.76) & 0.75 (0.75)\\ 
\verb!miniboone! & 130064 & 50 & 2 & 0.87 (0.87) & 0.87 (0.87) & 0.85 (0.85)\\ 
\verb!molec-biol-promoter! & 106 & 57 & 2 & 0.73 (0.63) & 0.50 (0.63) & 0.50 (0.55)\\ 
\verb!molec-biol-splice! & 3190 & 60 & 3 & 0.70 (0.70) & 0.69 (0.70) & 0.58 (0.58)\\ 
\verb!monks-1! & 556 & 6 & 2 & 0.85 (0.78) & 0.77 (0.80) & 0.79 (0.70)\\ 
\verb!monks-2! & 601 & 6 & 2 & 0.63 (0.59) & 0.63 (0.60) & 0.62 (0.57)\\ 
\verb!monks-3! & 554 & 6 & 2 & 0.90 (0.90) & 0.88 (0.89) & 0.83 (0.85)\\ 
\verb!mushroom! & 8124 & 21 & 2 & 1.00 (1.00) & 1.00 (1.00) & 1.00 (1.00)\\ 
\verb!musk-1! & 476 & 166 & 2 & 0.71 (0.69) & 0.73 (0.68) & 0.58 (0.60)\\ 
\verb!musk-2! & 6598 & 166 & 2 & 0.91 (0.92) & 0.93 (0.92) & 0.87 (0.89)\\ 
\verb!nursery! & 12960 & 8 & 5 & 0.89 (0.91) & 0.91 (0.91) & 0.84 (0.85)\\ 
\verb!oocytes_merluccius_nucleus_4d! & 1022 & 41 & 2 & 0.66 (0.68) & 0.70 (0.69) & 0.59 (0.65)\\ 
\verb!oocytes_merluccius_states_2f! & 1022 & 25 & 3 & 0.86 (0.86) & 0.85 (0.86) & 0.79 (0.83)\\ 
\verb!oocytes_trisopterus_nucleus_2f! & 912 & 25 & 2 & 0.65 (0.67) & 0.66 (0.67) & 0.62 (0.62)\\ 
\verb!oocytes_trisopterus_states_5b! & 912 & 32 & 3 & 0.86 (0.80) & 0.78 (0.80) & 0.78 (0.76)\\ 
\verb!optical! & 5620 & 62 & 10 & 0.76 (0.77) & 0.76 (0.78) & 0.64 (0.66)\\ 
\verb!ozone! & 2536 & 72 & 2 & 0.94 (0.95) & 0.95 (0.95) & 0.96 (0.94)\\ 
\verb!page-blocks! & 5473 & 10 & 5 & 0.93 (0.95) & 0.94 (0.95) & 0.93 (0.94)\\ 
\verb!parkinsons! & 195 & 22 & 2 & 0.77 (0.79) & 0.90 (0.79) & 0.77 (0.75)\\ 
\verb!pendigits! & 10992 & 16 & 10 & 0.92 (0.91) & 0.90 (0.91) & 0.88 (0.86)\\ 
\verb!pima! & 768 & 8 & 2 & 0.62 (0.67) & 0.69 (0.67) & 0.66 (0.65)\\ 
\verb!pittsburg-bridges-MATERIAL! & 106 & 7 & 3 & 0.73 (0.74) & 0.95 (0.77) & 0.73 (0.72)\\ 
\verb!pittsburg-bridges-REL-L! & 103 & 7 & 3 & 0.57 (0.55) & 0.57 (0.54) & 0.57 (0.48)\\ 
\verb!pittsburg-bridges-SPAN! & 92 & 7 & 3 & 0.55 (0.56) & 0.55 (0.57) & 0.50 (0.54)\\ 
\verb!pittsburg-bridges-T-OR-D! & 102 & 7 & 2 & 0.86 (0.81) & 0.95 (0.81) & 0.91 (0.81)\\ 
\verb!pittsburg-bridges-TYPE! & 105 & 7 & 6 & 0.71 (0.45) & 0.38 (0.44) & 0.38 (0.39)\\ 
\verb!planning! & 182 & 12 & 2 & 0.74 (0.57) & 0.61 (0.57) & 0.61 (0.58)\\ 
\verb!plant-margin! & 1600 & 64 & 100 & 0.24 (0.26) & 0.24 (0.26) & 0.10 (0.12)\\ 
\verb!plant-shape! & 1600 & 64 & 100 & 0.31 (0.28) & 0.24 (0.28) & 0.18 (0.17)\\ 
\verb!plant-texture! & 1599 & 64 & 100 & 0.36 (0.29) & 0.29 (0.29) & 0.14 (0.13)\\ 
\verb!post-operative! & 90 & 8 & 3 & 0.50 (0.53) & 0.28 (0.54) & 0.39 (0.58)\\ 
\verb!primary-tumor! & 330 & 17 & 15 & 0.36 (0.31) & 0.41 (0.29) & 0.23 (0.25)\\ 
\verb!ringnorm! & 7400 & 20 & 2 & 0.86 (0.85) & 0.84 (0.86) & 0.80 (0.79)\\ 
\verb!seeds! & 210 & 7 & 3 & 0.81 (0.85) & 0.83 (0.84) & 0.83 (0.83)\\ 
\verb!semeion! & 1593 & 256 & 10 & 0.55 (0.58) & 0.57 (0.58) & 0.41 (0.45)\\ 
\verb!soybean! & 683 & 35 & 18 & 0.74 (0.72) & 0.72 (0.72) & 0.65 (0.60)\\ 
\verb!spambase! & 4601 & 57 & 2 & 0.89 (0.87) & 0.88 (0.87) & 0.86 (0.83)\\ 
\verb!spect! & 265 & 22 & 2 & 0.57 (0.60) & 0.58 (0.60) & 0.72 (0.58)\\ 
\verb!spectf! & 267 & 44 & 2 & 0.75 (0.78) & 0.84 (0.78) & 0.73 (0.76)\\ 
\verb!statlog-australian-credit! & 690 & 14 & 2 & 0.48 (0.57) & 0.62 (0.57) & 0.53 (0.56)\\ 
\verb!statlog-german-credit! & 1000 & 24 & 2 & 0.62 (0.65) & 0.61 (0.65) & 0.59 (0.62)\\ 
\verb!statlog-heart! & 270 & 13 & 2 & 0.74 (0.67) & 0.72 (0.68) & 0.76 (0.64)\\ 
\verb!statlog-image! & 2310 & 18 & 7 & 0.93 (0.92) & 0.91 (0.92) & 0.89 (0.89)\\ 
\verb!statlog-landsat! & 6435 & 36 & 6 & 0.80 (0.82) & 0.83 (0.82) & 0.77 (0.78)\\ 
\verb!statlog-shuttle! & 58000 & 9 & 7 & 1.00 (1.00) & 1.00 (1.00) & 1.00 (1.00)\\ 
\verb!statlog-vehicle! & 846 & 18 & 4 & 0.64 (0.63) & 0.64 (0.63) & 0.46 (0.57)\\ 
\verb!steel-plates! & 1941 & 27 & 7 & 0.60 (0.61) & 0.63 (0.62) & 0.54 (0.55)\\ 
\verb!synthetic-control! & 600 & 60 & 6 & 0.85 (0.82) & 0.84 (0.82) & 0.74 (0.72)\\ 
\verb!teaching! & 151 & 5 & 3 & 0.48 (0.46) & 0.32 (0.45) & 0.32 (0.39)\\ 
\verb!thyroid! & 7200 & 21 & 3 & 0.98 (0.99) & 0.99 (0.98) & 0.98 (0.98)\\ 
\verb!tic-tac-toe! & 958 & 9 & 2 & 0.80 (0.81) & 0.82 (0.81) & 0.72 (0.72)\\ 
\verb!titanic! & 2201 & 3 & 2 & 0.76 (0.78) & 0.79 (0.78) & 0.91 (0.95)\\ 
\verb!trains! & 10 & 29 & 2 & 1.00 (0.48) & 1.00 (0.45) & 1.00 (0.47)\\ 
\verb!twonorm! & 7400 & 20 & 2 & 0.83 (0.82) & 0.83 (0.82) & 0.76 (0.75)\\ 
\verb!vertebral-column-2clases! & 310 & 6 & 2 & 0.77 (0.77) & 0.92 (0.76) & 0.76 (0.74)\\ 
\verb!vertebral-column-3clases! & 310 & 6 & 3 & 0.61 (0.75) & 0.73 (0.75) & 0.73 (0.71)\\ 
\verb!wall-following! & 5456 & 24 & 4 & 0.94 (0.94) & 0.97 (0.94) & 0.93 (0.91)\\ 
\verb!waveform! & 5000 & 21 & 3 & 0.73 (0.72) & 0.71 (0.71) & 0.65 (0.66)\\ 
\verb!waveform-noise! & 5000 & 40 & 3 & 0.67 (0.69) & 0.72 (0.69) & 0.63 (0.62)\\ 
\verb!wine! & 178 & 13 & 3 & 0.75 (0.84) & 0.89 (0.84) & 0.75 (0.77)\\ 
\verb!wine-quality-red! & 1599 & 11 & 6 & 0.48 (0.51) & 0.54 (0.52) & 0.45 (0.47)\\ 
\verb!wine-quality-white! & 4898 & 11 & 7 & 0.50 (0.49) & 0.48 (0.49) & 0.42 (0.42)\\ 
\verb!yeast! & 1484 & 8 & 10 & 0.43 (0.45) & 0.45 (0.46) & 0.42 (0.42)\\ 
\verb!zoo! & 101 & 16 & 7 & 1.00 (0.81) & 0.90 (0.81) & 0.90 (0.73)\\ 
\bottomrule 
\end{tabular} 

